A Case for Sustainability and Environment Friendliness in Software Development and Architecture Decisions by Taking Energy-Efficient Design Decisions

IT power usage is a significant concern. Data center energy consumption is estimated to account for 1% to 1.5% of all energy consumption worldwide. Hardware designers, data center designers, and other members of the IT community have been working to improve energy efficiency across many parts of the IT infrastructure; however, little attention has been paid to the energy efficiency of software components. Indeed, energy efficiency is currently not a common performance criteria for software. In this work, we attempt to quantify the potential for gains in energy efficiency in software, based on a set of examples drawn from common, everyday decisions made by software developers and enterprise architects. Our results show that there is potential for significant energy savings through energy-conscious choices at software development and selection time, making the software and IT artifact sustainable and environment friendly.

==> hold.tex <==

In this work, we consider the question of how members of the IS/IT community can operationalize this vision.~~Watson et al.~\cite{wbc:10} propose a starting point, where energy usage data are gathered via a sensor framework and provided to those stakeholders who can effect change and improve energy efficiency.  This raises the questions of how to gather the usage data, and who those stakeholders are. 

Basic energy usage statistics for a computer are not difficult to gather.  Since the power is drawn through the socket, we can place an energy usage monitor, such as the WattsUp?~\cite{wattsup:11} meter between the server's plug and the power source, and record data.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

current technology does not provide detailed energy usage statistics.  Without such a mapping, the availability of simple energy usage information provides no context for acting on that data in a software construction or enterprise architecture context

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
